Learning-based Adaptive Control using Contraction Theory

Adaptive control is subject to stability and performance issues when a learned model is used to enhance its performance. This paper thus presents a deep learning-based adaptive control framework for nonlinear systems with multiplicatively-separable parametrization, called adaptive Neural Contraction Metric (aNCM). The aNCM approximates real-time optimization for computing a differential Lyapunov function and a corresponding stabilizing adaptive control law by using a Deep Neural Network (DNN). The use of DNNs permits real-time implementation of the control law and broad applicability to a variety of nonlinear systems with parametric and nonparametric uncertainties. We show using contraction theory that the aNCM ensures exponential boundedness of the distance between the target and controlled trajectories in the presence of parametric uncertainties of the model, learning errors caused by aNCM approximation, and external disturbances. Its superiority to the existing robust and adaptive control methods is demonstrated using a cart-pole balancing model.

==> sections/old4_adaptiveNCM.tex <==
\section{Adaptive Neural Contraction Metrics}
\label{ancm}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We introduce an adaptive Neural Contraction Metrics (aNCM) for designing a real-time implementable control policies with asymptotic stability, for a variety of parametric uncertain nonlinear systems.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Affine Parameter Uncertainty}
We first consider the following systems:
\begin{align}
\label{adaptive_affine}
\dot{x} =& f(x,t)+B(x,t)u-\Delta(x,t)^{\top}\theta \\
\label{adaptive_affine_d}
\dot{x}_d =& f(x_d,t)+B(x_d,t)u_d-\Delta(x_d,t)^{\top}\theta
\end{align}
where $\theta\in\mathbb{R}^p$, $\Delta:\mathbb{R}^n\times\mathbb{R}_{\geq0}\mapsto\mathbb{R}^{n\times p}$, and the other variables are as defined in (\ref{sdc_dynamics}). For these systems with the matched uncertainty condition, the modified NCM in Theorem~\ref{modified_ncm_thm} can be augmented to its adaptive counterpart.
\begin{theorem}
\label{adaptive_affine_thm}
Suppose that $f$ and $B$ in (\ref{adaptive_affine}) are continuously differentiable, and we have $M(x,x_d,t)$ given by (\ref{convex_opt_ncm}) in Theorem~\ref{modified_ncm_thm} for the nominal system (\ie{} (\ref{adaptive_affine}) and (\ref{adaptive_affine_d}) with $\Delta=0,\forall x,t$). If the matched uncertainty condition holds, \ie{} $(\Delta(x,t)-\Delta(x_d,t))^{\top}\theta \in \text{span}(B(x,t))$, then the following adaptive control law guarantees asymptotic stability of (\ref{adaptive_affine}):
\begin{align}
\label{affine_adaptive_u}
u =& u_d-B(x,t)^{\top}M(x,x_d,t)(x-x_d)+\varphi(x,x_d,t)^{\top} \hat{\theta} \\
\label{affine_adaptation}
\dot{\hat{\theta}} =& -\Gamma \varphi(x,x_d,t)B(x,t)^{\top}M(x,x_d,t)(x-x_d)
\end{align}
where $\Gamma \succ 0$ and $(\Delta(x,t)-\Delta(x_d,t))^{\top}\theta=B(x,t)\varphi(x,x_d,t)^{\top}\theta$.
\end{theorem}
\begin{proof}
Let $A_{cl}=A(x,x_d,t)-B(x,t)B(x,t)^{\top}M(x,x_d,t)$. The virtual system of (\ref{adaptive_affine}), (\ref{adaptive_affine_d}), and (\ref{affine_adaptation}) with (\ref{affine_adaptive_u}), which has $(x,\hat{\theta})$ and $(x_d,\theta)$ as its particular solutions, is given as 
\begin{align}
\label{affine_q1}
\dot{q}_1 =& \dot{x}_d+A_{cl}(q_1-x_d)+B(x,t)\varphi(x,x_d,t)^{\top}(q_2-\theta) \\
\label{affine_q2}
\dot{q}_2 =& -\Gamma \varphi(x,x_d,t)B(x,t)^{\top}M(x,x_d,t)(q_1-x_d).
\end{align}
where $\tilde{\Delta}=\Delta(x,t)-\Delta(x_d,t)$ and the relation $\tilde{\Delta}^{\top}\theta=B(x,t)\varphi(x,x_d,t)^{\top}\theta$ is used. Thus for a Lyapunov function defined as $V = \delta q_1^{\top}M(x,x_d,t)\delta q_1+\delta q_2^{\top}\Gamma^{-1}\delta q_2$, we have $\dot{V} \leq -2\alpha \delta q_1^{\top}M\delta q_1+2\delta q_1^{\top}MB\varphi^{\top}\delta q_2+2\delta q_2^{\top}\Gamma^{-1}\delta \dot{q}_2$ by the proof of Theorem~\ref{modified_ncm_thm}. Thus, (\ref{affine_adaptation}) gives $\dot{V} \leq -2\alpha \delta q_1^{\top}M\delta q_1$, which implies asymptotic stability of (\ref{adaptive_affine})~\cite{Slotine:1228283}.
\end{proof}
\begin{corollary}
\label{adaptive_affine_thm_cor}
The controller (\ref{affine_adaptive_u}) with the adaptation law
\begin{align}
\dot{\hat{\theta}} =& -\Gamma \varphi(x,x_d,t)B(x,t)^{\top}M(x,x_d,t)(x-x_d)-\alpha (\hat{\theta}-\theta_n)
\end{align}
where $\theta_n$ is a guess for the true parameter $\theta$, gives the following exponential bound on the tracking error:
\begin{align}
\label{adaptive_exponential_affine}
\|x-x_d\| \leq \sqrt{\frac{V(x(0),x_d(0))}{\underline{\rho}}}e^{- \alpha t}+\sqrt{\frac{\overline{\rho}}{\underline{\rho}}}{\|\theta-\theta_n\|}.
\end{align}
where $\underline{\rho},\overline{\rho}>0$ with $\underline{\rho}I\preceq \text{diag}(M,\Gamma^{-1})\preceq\overline{\rho}I$.
\end{corollary}
\begin{proof}
Consider the virtual system (\ref{affine_q1}), and (\ref{affine_q2}) with an additional term $-\alpha (q_2-\theta)+d(q_2)$, where $d(\hat{\theta})=\alpha (\theta_n-\theta)$ and $d(\theta)=0$.
For $V = \delta q_1^{\top}M(x,x_d)\delta q_1+\delta q_2^{\top}\Gamma^{-1}\delta q_2$, we have $\dot{V}\leq -2\alpha V+2\delta q_2^{\top}\Gamma^{-1}d$ by Theorem~\ref{adaptive_affine_thm}, and thus $\dot{R} \leq-\alpha R(t)+\alpha\sqrt{\overline{\rho}}\|\theta_n-\theta\|$, for $R(t)=\|\Theta (x(t),x_d(t),t)\|\delta q (t)$ with $q = [q_1^{\top},q_2^{\top}]^{\top}$ and $\text{diag}(M,\Gamma^{-1})=\Theta^{\top}\Theta$. Applying the comparison lemma~\cite{Khalil:1173048} results in (\ref{adaptive_exponential_affine}).
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Modified NCM for Lagrangian-type Nonlinear Systems}
We have thus far examined the case where $f(x,t)$ is affine in its parameters. This section considers the following dynamical system with uncertain parameters $\theta$ and a control input $\tau$:
\begin{align}
\label{lagrangian_dynamics}
H(s,t)\dot{s}+h(s,t)+\Delta(s,t)\theta = \tau
\end{align}
where $s\in \mathbb{R}^n$, $\tau\in \mathbb{R}^n$, $H:\mathbb{R}^{n}\times\mathbb{R}_{\geq 0}\mapsto \mathbb{R}^{n\times n}$, $h:\mathbb{R}^{n}\times\mathbb{R}_{\geq 0}\mapsto \mathbb{R}^{n}$, $\Delta:\mathbb{R}^{n}\times\mathbb{R}_{\geq 0}\mapsto \mathbb{R}^{n\times p}$, and $H(s,t)$ is non-singular for all $s,t$. We often encounter the problem of designing a controller with an asymptotic convergence guarantee ($s\to0$), one example of which is the tracking control of Lagrangian systems~\cite{Slotine:1228283}. The modified NCM is also applicable to such problems due to the following corollary.
\begin{corollary}
\label{lagrangian_NCM}
Let $M(s,t)$ be an NCM for the dynamical system $\dot{s}=-H(s,t)^{-1}h(s,t)+H(s,t)^{-1}\tau$ given by (\ref{convex_opt_ncm}) of Theorem~\ref{modified_ncm_thm}. If we design $\tau$ as
\begin{align}
\label{lagrange_control}
\tau =& -H(s,t)^{-\top}M(s,t)s+\Delta (s,t)\hat{\theta} \\
\label{lagrange_adaptation}
\dot{\hat{\theta}} =& -\Gamma\Delta (s,t)^{\top}H(s,t)^{-\top}M(s,t)s
\end{align}
then $s$ of (\ref{lagrangian_dynamics}) asymptotically converges to $0$.
\end{corollary}
\begin{proof}
Similar to Theorem~\ref{adaptive_affine_thm}, the virtual system is expressed as $H\dot{q}_1+h=-H^{-1}Mq_1+\Delta (q_2-\theta)$ and $\dot{q}_2=-\Gamma\Delta^{\top}H^{-\top}M q_1$.
Thus for $V = \delta q_1^{\top}M\delta q_1+\delta q_2^{\top}\Gamma^{-1}\delta q_2$, we have $\dot{V}/2\leq-\alpha \delta q_1^{\top}M\delta q_1+\delta q_1^{\top}MH^{-1}\Delta\delta q_2+\delta q_2^{\top}\Gamma^{-1}\delta \dot{q}_2$. Thus, (\ref{lagrange_adaptation}) gives $\dot{V}\leq-2\alpha \delta q_1^{\top}M\delta q_1$ as desired.
\end{proof}
\begin{remark}
An exponential boundedness result similar to Corollary~\ref{adaptive_affine_thm_cor} is obtainable with the adaptation law $\dot{\hat{\theta}} = -\Gamma\Delta (s,t)^{\top}H(s,t)^{-\top}M(s,t)s-2\alpha(\hat{\theta}-\theta_n)$, where $\theta_n$ is a nominal guess of $\theta$.
\end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Multiplicatively Separable Parameter Uncertainty}
Next, let us consider the following nonlinear system with uncertain parameters $\theta\in\mathbb{R}^p$:
\begin{align}
\label{adaptive_general}
\dot{x} = f(x,t;\theta)+B(x,t;\theta)u,~\dot{x}_d = f(x_d,t;\theta)+B(x_d,t;\theta)u_d.
\end{align}
In this section, we assume the following.
\begin{assumption}
\label{multiplicative_asmp}
The system (\ref{adaptation_general}) is multiplicatively separable in terms of $x,t$ and $\theta$, \ie{}, $\exists$ $Y_f:\mathbb{R}^n\times\mathbb{R}_{\geq0}\mapsto\mathbb{R}^{n\times q_z}$, $Y_{b_i}:\mathbb{R}^n\times\mathbb{R}_{\geq0}\mapsto\mathbb{R}^{m\times q_z},\forall i$, and $Z:\mathbb{R}^p\mapsto\mathbb{R}^{q_z}$ \st{} 
\begin{align}
\label{linear_adaptive}
Y_f(q,t)Z(\theta) = f(q,t;\theta),~Y_{b_i}(q,t)Z(\theta) = b_i(q,t;\theta)
\end{align}
where $B(x,t;\theta)=[b_1(x,t;\theta),\cdots,b_n(x,t;\theta)]^{\top}$. 
\end{assumption}
\begin{remark}
When Assumption~\ref{multiplicative_asmp} holds, we could always redefine $\theta$ as $[\theta^{\top},Z(\theta)^{\top}]^{\top}$ to have $Y_f(q,t)\theta = f(q,t;\theta)$ and $Y_{b_i}(q,t)\theta = b_i(q,t;\theta)$. Since we can implicitly regularize such an over-parameterized systems using the Bregman divergence as will be seen in Corollary~\ref{implicit_reg_thm}, we denote $[\theta^{\top},Z(\theta)^{\top}]^{\top}$ as $\theta$ in the subsequent discussion.
\end{remark}

Under Assumption~\ref{multiplicative_asmp} with $\theta$ augmented as $[\theta^{\top},Z(\theta)^{\top}]^{\top}$, the error dynamics for $e=x-x_d$ of (\ref{adaptive_general}) can be expressed as follows: 
\begin{align}
\label{error_dynamics}
\dot{e} =& A(x,x_d,t;\hat{\theta})e+B(x,t;\hat{\theta})(u-u_d)-\tilde{Y}(\hat{\theta}-\theta) \\
\label{definition_Y}
\tilde{Y} =& Y-Y_d= (Y_f(x,t)+Y_b(x,u,t))-(Y_f(x_d,t)+Y_b(x_d,u_d,t))
\end{align}
where $Y_b(x,u,t)=[Y_{b_1}(x,t)^{\top}u,\cdots,Y_{b_n}(x,t)^{\top}u]^{\top}$, $A$ is the SDC matrix defined in Lemma~\ref{sdclemma}, and $\hat{\theta}$ is the current estimate of $\theta$. The following theorem presents the NCM-based adaptive control for asymptoric stabilization of (\ref{error_dynamics}).
%\begin{remark}
%Note that the conditions (\ref{linear_adaptive}) and (\ref{linear_adaptive2}) are not strict in a sense that we can always over-parameterize the system, and the adaptation law with the Bregman divergence~\cite{boffi2020implicit} will give us some insight on the implicit regularization on these parameters, which could circumvent the issue of overfitting.
%\end{remark}
%\begin{example}
%For $f(x;\theta) = x_1\theta+x_3^2\theta^2+x_2^3\cos\theta$, we have
%\begin{align}
%f(x;\theta) = [x_1~x_3^2~x_2^3]\begin{bmatrix}\theta_{\max} & 0 & 0\\0 & \theta_{\max}^2 & 0 \\ 0 & 0 & 1\end{bmatrix}\begin{bmatrix}\theta/\theta_{\max}\\\theta^2/\theta_{\max}^2 \\ \cos\theta\end{bmatrix}
%\end{align}
%so we can use $\bar{\theta} = [\theta/\theta_{\max}~\theta^2/\theta_{\max}^2~\cos\theta]^{\top}$ as the unknown parameter.
%\end{example}
\begin{theorem}
\label{adaptiveNCMthm}
Suppose that Assumption~\ref{multiplicative_asmp} holds and let $B=B(x,t;\hat{\theta})$ and $A=A(x,x_d,t;\hat{\theta})$ be the SDC matrix given in (\ref{error_dynamics}) for notational simplicity. Consider a neural network trained to perfectly model the optimal contraction metric $M(x,x_d,\hat{\theta},t)=W(x,x_d,\hat{\theta},t)^{-1}$ (we call such $M$ an adaptive Neural Contraction Metric (aNCM)), given by the following convex optimization problem:
\begin{align}
    \label{convex_opt_ancm}
    &{J}_{aCV}^* = \min_{\chi \in \mathbb{R},\bar{W}\succ 0} \frac{\overline{d}\chi}{\alpha} \text{~~\st{} (\ref{deterministic_contraction_adaptive_tilde}) and (\ref{adaptive_W_tilde})}.
\end{align}
with the convex constraints (\ref{deterministic_contraction_adaptive_tilde}) and (\ref{adaptive_W_tilde}) given as
\begin{align}
\label{deterministic_contraction_adaptive_tilde}
&-\left.\frac{d}{dt}\right|_{\hat{\theta}}{\bar{W}}+2\sym{\left(A\bar{W}\right)}-2\nu BB^{\top} \preceq -2\alpha \bar{W},~\forall x,x_d,\hat{\theta},t \\
\label{adaptive_W_tilde}
&I \preceq \bar{W}(x,x_d,\hat{\theta}) \preceq \chi I,~\forall x,x_d,\hat{\theta},t
\end{align}
where $\alpha,\underline{\omega},\overline{\omega} > 0$, $\chi = \overline{\omega}/\underline{\omega}$, $\bar{W} = \nu W$, $\nu = 1/\underline{\omega}$, and $({d}/{dt})|_{\hat{\theta}}{\bar{W}}$ is the time derivative of $\bar{W}$ computed along the dynamical system (\ref{adaptive_general}) with $\theta = \hat{\theta}$. If the true dynamics (\ref{adaptive_general}) is controlled by
\begin{align}
\label{adaptive_general_u}
u =& u_d-B(x,t;\hat{\theta})^{\top}M(x,x_d,\hat{\theta},t)(x-x_d)\\
\label{adaptation_general}
\dot{\hat{\theta}} =& \Gamma^{-1}(Y^{\top}dM_x+Y_d^{\top}dM_{x_d}+\tilde{Y}^{\top}M) (x-x_d)
\end{align}
where $dM_q = [({\partial M}/{\partial q_1})e,\cdots,({\partial M}/{\partial q_n})e]^{\top}/2$, $e=x-x_d$, $\Gamma \succ 0$, and $Y$, $Y_d$, $\tilde{Y}$ are as defined in (\ref{definition_Y}), then $e$ of (\ref{error_dynamics}) asymptotically converges to $0$. Also, when $\theta$ in (\ref{adaptive_general}) is given, the Euclidean distance between $x_d$ and $x$ with bounded disturbance and $x_d$ is exponentially bounded, and the metric $M$ minimizes its steady-state upper bound.
\end{theorem}
\begin{proof}
%The virtual system of (\ref{adaptive_general}) and (\ref{adaptation_general}) with (\ref{adaptive_general_u}), which has $(x,\theta)$ and $(x_d,\hat{\theta})$ as its particular solutions is given as
%\begin{align}
%\label{virtual_q1_general}
%\dot{q}_1 =& \dot{x}_d+A_{cl}(q_1-x_d)-\tilde{Y}(q_2-\theta) \\
%\label{virtual_q2_general}
%\dot{q}_2 =& \Gamma^{-1}(Y^{\top}dM_x(e)+Y_d^{\top}dM_{x_d}(e)+\tilde{Y}^{\top}M) (q_1-x_d)
%\end{align}
%where $A_{cl}=A(x,x_d,t;\hat{\theta})-B(x,t;\hat{\theta})B(x,t;\hat{\theta})^{\top}M(x,x_d,\hat{\theta},t)$.
Computing $\dot{M}e$ along the true dynamics (\ref{adaptive_general}) yields
\begin{align}
\dot{M}e=\left(\left.\frac{d}{dt}\right|_{\hat{\theta}}M\right)e-2(dM_x^{\top}Y+dM_{x_d}^{\top}Y_d)\tilde{\theta}
\end{align}
where $({d}/{dt})|_{\hat{\theta}}{M}$ is the time derivative of $M$ computed along \ref{adaptive_general}) with $\theta = \hat{\theta}$. Thus for $V = e^{\top}Me+\tilde{\theta}^{\top}\Gamma\tilde{\theta}$, we have
$\dot{V} \leq -2\alpha e^{\top}Me-2e^{\top}(dM_x^{\top}Y+dM_{x_d}^{\top}Y_d+M\tilde{Y})\tilde{\theta}+\tilde{\theta}^{\top}\Gamma\dot{\tilde{\theta}}$ by (\ref{error_dynamics}), (\ref{adaptive_general_u}), and Theorem~\ref{modified_ncm_thm} along with (\ref{deterministic_contraction_adaptive_tilde}) and (\ref{adaptive_W_tilde}). The adaptation law (\ref{adaptation_general}) applied to this relation gives $\dot{V} \leq -2\alpha e^{\top}Me$, which implies asymptotic stability of (\ref{error_dynamics}). The final statement on optimality of $M$ follows by Theorem~\ref{modified_ncm_thm}.
{\color{caltechorange} HAS TO APPLY BARBALAT LEMMA OR USE DIFFERENTIAL DYNAMICS}
\end{proof}

We could also incorporate the Bregman divergence-based implicit regularization on its parameter convergence~\cite{boffi2020implicit} using the following Corollary.
\begin{corollary}
\label{implicit_reg_thm}
Let $\psi:\mathbb{R}^p\mapsto\mathbb{R}$ be a given convex function and consider an adaptive controller (\ref{adaptive_general_u}) for (\ref{adaptation_general}) with the following adaptation law 
\begin{align}
\label{adaptation_general_bregman}
\dot{\hat{\theta}} =& (\nabla^2\psi(\hat{\theta}))^{-1}(Y^{\top}dM_x+Y_d^{\top}dM_{x_d}+\tilde{Y}^{\top}M) (x-x_d).
\end{align}
Then $e$ of (\ref{error_dynamics}) asymptotically converges to $0$. Also, suppose that $\theta^*=\lim_{t\to \infty}\hat{\theta}(t)\in A$, where $A=\{\vartheta|\Xi(t)^{\top}\vartheta=\Xi(t)^{\top}\theta,\forall t\}$ for the true parameter $\theta$ with $\Xi(\tau) = (Y^{\top}dM_x+Y_d^{\top}dM_{x_d}+\tilde{Y}^{\top}M)|_{t=\tau}$. Then we have
\begin{align}
\label{implicit_reg}
\theta^*=\text{arg}\min_{\vartheta\in A}d_{\psi}(\vartheta\|\theta^*)=\text{arg}\min_{\vartheta\in A}d_{\psi}(\vartheta\|\hat{\theta}(0))
\end{align}
where $d_{\psi}$ is the Bregman divergence defined as $d_{\psi}(x\|y)=\psi(x)-\psi(y)-(x-y)^{\top}\nabla\psi(y)$. Further, selecting $\hat{\theta}(0)$ as $\hat{\theta}(0)=\text{arg}\min_{b\in \mathbb{R}^p}\psi(b)$ yields $\theta^*=\text{arg}\min_{\vartheta\in A}\psi(\vartheta)$.
\end{corollary}
\begin{proof}
Asymptotic stability follows by the proof of Theorem~\ref{adaptive_affine_thm} applied to $V = e^{\top}Me+2d_{\psi}(\theta|\hat{\theta})$ with the the property of the Bregman divergence $d(d_{\psi}(\theta\|\hat{\theta}))/dt = (\hat{\theta}-\theta)^{\top}\nabla^2\psi(\hat{\theta})\dot{\hat{\theta}}$ with (\ref{adaptation_general_bregman}). Next, we have for any $\vartheta \in A=\{\vartheta|\Xi(t)^{\top}\vartheta=\Xi(t)^{\top}\theta,\forall t\}$ that
\begin{align}
d_{\psi}(\vartheta\|\theta^*)-d_{\psi}(\vartheta\|\hat{\theta}(0))=\int^\infty_0(\hat{\theta}(\tau)-\theta)^{\top}\Xi(\tau)e(\tau)d\tau \nonumber
\end{align}
where $\Xi(\tau) = (Y^{\top}dM_x+Y_d^{\top}dM_{x_d}+\tilde{Y}^{\top}M)|_{t=\tau}$. Since the right hand side does not depend on $\vartheta$ and its minimum over $\vartheta \in A$ is clearly obtained at $\theta^*\in A$, we have (\ref{implicit_reg}) as desired. Also, $\hat{\theta}(0)=\text{arg}\min_{b\in \mathbb{R}^p}\psi(b)$ implies $\nabla\psi(\hat{\theta}(0))=0$ by the convexity of $\psi$, resulting in $d_{\psi}(\vartheta\|\hat{\theta}(0))=\psi(\vartheta)$.
{\color{caltechorange} HAS TO APPLY BARBALAT LEMMA OR USE DIFFERENTIAL DYNAMICS}
\end{proof}
\begin{remark}
An important example of $\psi$ in (\ref{implicit_reg_thm}) is a norm, which could regularize the unknown parameters implicitly by (\ref{implicit_reg}). The choice of norms leads to different properties of the steady-state estimated parameters such as sparsity~\cite{boffi2020implicit}.
\end{remark}
\begin{remark}
Adding the decaying term $-2\alpha (\hat{\theta}-\theta_n)$ with the nominal parameters $\theta_n$ to the adaptation laws (\ref{adaptation_general}) and (\ref{adaptation_general_bregman}) again leads to exponential boundedness of the tacking error as in Corollary~\ref{adaptive_affine_thm_cor}, which could be more useful than asymptotic convergence in practical applications.
\end{remark}

==> sections/old_applications.tex <==
\section{Practical Application of aNCM Control}
\label{applications}
This section delineates how to apply the aNCM control law to several important engineering and robotics examples, and proposes practical numerical algorithms to construct aNCMs using Theorem~\ref{adaptive_affine_thm}~and~\ref{adaptiveNCMthm}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Systems Modeled by Function Approximators}
Utilization of function approximators, neural networks in particular, has gained great popularity in system identification due to their high representational power, and provably  stable techniques for using
these approximators in closed-loop have been derived in~\cite{SannerSlotine1992}. The aNCM framework can also be used to guarantee asymptotic stability and exponential boundedness of system trajectories in this context.

Consider the following system with basis functions 
$\phi(x)=[\phi_1(x),\cdots,\phi_p(x)]^{\top}$ and 
$\varphi_i(x)=[\varphi_{i,1}(x),\cdots,\varphi_{i,q}(x)]^{\top}$, $i=1,\cdots,m$, which approximate $f(x)$ and $B(x)=[b_1(x),\cdots,b_m(x)]$ of the true dynamical system, respectively:
\begin{align}
\label{basis_func_dyn}
\dot{x} = f(x)+B(x)u \simeq \mathcal{F}\phi(x)+\sum_{i=1}^m\mathcal{B}_i\varphi_i(x)u_i
\end{align}
where $\mathcal{F}\in\mathbb{R}^{n\times p}$, $\mathcal{B}_i\in\mathbb{R}^{n\times q}$, $\mathcal{F}\phi(x)\simeq f(x)$, and $\mathcal{B}_i\varphi_i(x)\simeq b_i(x)$. The following proposition introduces aNCM-based adaptation laws to update the weights $\mathcal{F}$ and $\mathcal{B}_i$ for asymptotic stabilization.
\begin{proposition}
\label{basis_function_prop}
Suppose $\exists \mathcal{F}^*$ and $\mathcal{B}^*_i$ \st{} $\mathcal{F}^*\phi(x) = f(x)$ and $\mathcal{B}_i^*\varphi_i(x) = b_i(x),\forall i,~\forall x \in \mathbb{R}^n$. Let $M(x,x_d,\hat{\mathcal{F}},\hat{\mathcal{B}})$ be the aNCM for \eqref{basis_func_dyn} given by \eqref{convex_opt_ancm} with the same assumptions of Theorem~\ref{adaptiveNCMthm}, where $\hat{\mathcal{F}}$ and $\hat{\mathcal{B}}$ are the estimates of $\mathcal{F}^*$ and $\mathcal{B}^*$. Also, let $\mathcal{W}$ denote the weights, and let $\zeta=\phi(x)$ and $\zeta_d=\phi(x_d)$ for $\mathcal{W}=\mathcal{F}$, and $\zeta=\varphi_i(x)u_i$ and $\zeta_d=\varphi_i(x_d)u_{d,i}$ for $\mathcal{W}=\mathcal{B}_i$. If $u$ is given by \eqref{adaptive_general_u}, the following adaptation
\begin{align}
\label{adaptation_F}
\dot{\hat{\mathcal{W}}} = (\nabla^2\psi(\hat{\mathcal{W}}))^{-1}\textbf{:} (dM_xe\zeta^{\top}+dM_{x_d}e\zeta_{d}^{\top}+Me\tilde{\zeta}^{\top})
\end{align}
where $\tilde{\zeta}=\zeta-\zeta_{d}$ and $\textbf{:}$ is defined as $(A\textbf{:}B)_{ij}=\sum_{k,\ell}A_{ijk\ell}B_{\ell k}$, %(for $A\in \mathbb{R}^{n\times m \times p \times q}$, $B\in \mathbb{R}^{q \times p}$),
guarantees asymptotic convergence of $e=x-x_d$ to $0$ for \eqref{basis_func_dyn}. Note that $\nabla^2\psi(\cdot)$ represents the fourth order tensor given as $\nabla^2\psi(\cdot)_{ijk\ell}=\partial^2 \psi/(\partial(\cdot)_{ij}\partial(\cdot)_{\ell k})$ for a convex function $\psi(\cdot)$. Further, $\hat{\mathcal{F}}$ and $\hat{\mathcal{B}}_i$ are implicitly regularized by $\psi$ when they converge to the true parameter in the sets $\{\vartheta|M(\mathcal{W}^*-\vartheta)\tilde{\zeta}+dM_{x}^{\top}(\mathcal{W}^*-\vartheta)\zeta+dM_{x_d}^{\top}(\mathcal{W}^*-\vartheta)\zeta_{d}=0\}$. Adding the decaying term to \eqref{adaptation_F} leads to exponential boundedness of the tracking error as in Corollary~\ref{adaptiveNCMcor}.
\end{proposition}
\begin{proof}
Let us define $V$ as $V = 2\sum_{\mathcal{W}=\mathcal{F},\mathcal{B}_i}d_{\psi}(\mathcal{W}^*|\hat{\mathcal{W}})+e^{\top}Me$, where $d_{\psi}(\theta\|\hat{\theta})=\psi(\theta)-\psi(\hat{\theta})+(\hat{\theta}-\theta)\textbf{:}(\nabla\psi(\hat{\theta}))$. Also, let $V_e=e^{\top}Me$ and $\tilde{\mathcal{W}}=\hat{\mathcal{W}}-\mathcal{W}^*$. Since $M$ is the aNCM of \eqref{deterministic_contraction_adaptive_tilde}, we have as in the proof of Theorem~\ref{adaptiveNCMthm} that $\dot{V}_e \leq -2\alpha e^{\top}Me-2e^{\top}\sum_{\mathcal{W}=\mathcal{F},\mathcal{B}_i}(dM_x^{\top}\tilde{\mathcal{W}}\zeta+dM_{x_d}^{\top}\tilde{\mathcal{W}}\zeta_{d}+M\tilde{\mathcal{W}}\tilde{\zeta})$. This along with \eqref{adaptation_F} gives $\dot{V} \leq -2\alpha e^{\top}Me$ due to $a^{\top}Cb=C\textbf{:}(ab^{\top})$ for $a\in\mathbb{R}^n$, $b\in\mathbb{R}^p$, and $C\in\mathbb{R}^{n\times p}$. The regularization statement follows from Corollary~\ref{implicit_reg_thm}.
\end{proof}

We can utilize the same technique for neural net modeled systems to adaptively update the weights of its last layer.
\begin{corollary}
\label{adaptiveNCMthm_NN}
Consider the following system, $\dot{x} = f
(x)+B(x)u = \mathcal{F}^*\varrho(x;\mathcal{F}_{1:L})+\sum_{i=1}^m\mathcal{B}_i^*\beta_{i}(x;\mathcal{B}_{1:L}^{(i)})u_i$, where $\varrho$ and $\beta_{i}$ are the nominal neural nets with the trained weights of the first $L$ layers, $\bar{\mathcal{F}}_{1:L}$ and $\bar{\mathcal{B}}_{1:L}^{(i)}$, and $\mathcal{F}^*$ and $\mathcal{B}_i^*$ are the true weights of their last layers. Then the aNCM control \eqref{adaptive_general_u} under the adaptation law \eqref{adaptation_F} with $\phi(x)$ and $\varphi_i(x)$ replaced by $\rho(x;\mathcal{F}_{1:L})$ and $\beta_i(x;\mathcal{B}_{1:L}^{(i)})$, respectively, guarantees asymptotic convergence of $e=x-x_d$ to $0$.
\end{corollary}
\begin{proof}
See the proof of Proposition~\ref{basis_function_prop}.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Additional Remarks in aNCM Implementation}
We finally propose several useful implementation techniques for the practical application of the aNCM framework introduced in Theorem~\ref{adaptive_affine_thm}~and~\ref{adaptiveNCMthm}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Backward Approximation of Time Derivatives}
The construction of $M$ by \eqref{convex_opt_ncm} and \eqref{convex_opt_ancm} requires computation of $\dot{W}$ and $(d/dt)|_{\hat{\theta}}W$, respectively. One way to solve them as a finite-dimensional problem is to apply $\dot{\tilde{W}}(x(t_i),t_i) \simeq {({\tilde{W}}(x(t_i),t_i)-{\tilde{W}}(x(t_{i-1}),t_{i-1}))}/{\Delta t_i}$, where $\Delta t = t_i-t_{i-1}, \forall i$ with $\Delta t \gg \Delta t^2 > 0$  by using backward difference approximation on $\dot{\bar{W}}$, where we can then use $-\bar{W} \preceq -I$ to obtain a sufficient condition of its constraints. We could also solve it along pre-computed trajectories~(see \cite{ncm,nscm,doi:10.1162/neco.1997.9.8.1735} for details).
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Constraints as Loss Functions}
Instead of solving \eqref{convex_opt_ncm} and \eqref{convex_opt_ancm} for $\bar{W}$ to sample training data $\{(x,x_d,M)\}_{i=1}^N$, we could directly solve them for the neural net weights treating the constraints as loss functions for stochastic gradient descent in the network training. Since it is challenging to optimize the weights from scratch, we could initialize them with the solution given by the NCM~\cite{ncm}, and use spectral normalization~\cite{miyato2018spectral,nscm,8794351} to regularize the network for bounding $\partial M/\partial q$ (\ie{} $M$: Lipschitz),  where $q=x,x_d,\hat{\theta}$.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{aNCMs with Control Lyapunov Functions}
The aNCM can also be utilized as a Control Lyapunov Function (CLF)~\cite{lagros}. In particular, we consider a controller $u=u_d(x_d)+K^*(x,x_d)e$ in \eqref{adaptive_general}, where $K^*$ is given by
\begin{align}
\label{ancm_robust_control}
&K^* = \text{arg}\min_{K\in \mathbb{R}^{m\times n}}\|u-u_d(x_d)\|^2 = \text{arg}\min_{K\in \mathbb{R}^{m\times n}}\|K(x,x_d)e\|^2 \\
\label{stability_clf}
&\text{\st{} } \left.({d}/{dt})\right|_{\hat{\theta}}{M}+2\sym{}(MA+MK(x,x_d)) \leq -2\alpha M.
\end{align}
which is convex when $(x,x_d)$ is given at time $t$.
\begin{proposition}
If $M$ of \eqref{convex_opt_ancm} in Theorem~\ref{adaptiveNCMthm} is perfectly modeled by a neural net, \eqref{ancm_robust_control} is always feasible, \ie{}, $V=e^{\top}Me$ is a CLF for $e=x-x_d$, and minimizes the deviation of $u$ from $u_d(x_d)$ under the stability constraint \eqref{stability_clf}. Further, $u=u_d(x_d)+K^*e$ guarantees asymptotic stabilization of $e$ to $0$.
\end{proposition}
\begin{proof}
See~\cite{lagros}.
\end{proof}
\begin{remark}
For not perfectly modeled $M$, the optimization-based controller \eqref{ancm_robust_control} can be modified to guarantee its feasibility by rewriting the objective as $\|Ke\|^2+p^2$ and \eqref{stability_clf} as $({d}/{dt})|_{\hat{\theta}}{M}+2\sym{}(MA+MK) \leq -2\alpha M+p$, where $p$ is a decision variable to relax the stability constraint \eqref{stability_clf}. Convex input constraints can be incorporated by using the same relaxation technique.
\end{remark}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\if0
\subsection{aNCM Observer}
Let us consider the state estimation problem for the following nonlinear system with bounded disturbances:
\begin{align}
    \label{orig_dynamics_est}
    \dot{x} =& f(x,\theta)+B(x,\theta)d_1(t) \\
    \label{measurement_eq}
    y(t) =& h(x,\theta)+G(x,\theta)d_2(t)
\end{align}
where $d_1: \mathbb{R}_{\geq 0} \to \mathbb{R}^{k_1}$, $B:\mathbb{R}^n\times\mathbb{R}_{\geq 0} \to \mathbb{R}^{n\times k_1}$, $y: \mathbb{R}_{\geq 0} \to \mathbb{R}^m$, $d_2: \mathbb{R}_{\geq 0} \to \mathbb{R}^{k_2}$, $h:\mathbb{R}^n\times\mathbb{R}_{\geq 0} \to \mathbb{R}^{m}$, and $G:\mathbb{R}^n\times\mathbb{R}_{\geq 0} \to \mathbb{R}^{m\times k_2}$ with  $\overline{d}_1 = \sup_t\|d_1(t)\| < +\infty$ and $\overline{d}_2 = \sup_t\|d_2(t)\|  < +\infty$. We design an observer as 
\begin{align}
\label{estimator}
&\dot{\hat{x}} = f(\hat{x},\hat{\theta})+M(\hat{x},\hat{\theta})C_L(\hat{x},\hat{\theta})^{\top}(y-h(\hat{x},\hat{\theta})) \\
\label{estimator_con1}
&\dot{W}+2\sym(W A-C^{\top}_LC) \preceq -2\alpha W \\
\label{estimator_con2}
&\underline{\omega}I \preceq W(\hat{x},\hat{\theta}) \preceq \overline{\omega}I,~\forall x,\hat{x},\hat{\theta}
\end{align}
where $W = M(\hat{x},\hat{\theta})^{-1} \succ 0$, $\hat{\theta}$ is the estimate of $\theta$, $A(x,\hat{x},\theta)$ and $C(x,\hat{x},\theta)$ are given by \eqref{sdcAc} of Lemma~\ref{sdclemma} with $(f,x,x_d,u_d)$ replaced by $(f,\hat{x},x,0)$ and $(h,\hat{x},x,0)$, respectively, and $C_L(\hat{x},\hat{\theta})=C(\hat{x},\hat{x},\hat{\theta})$.
\begin{theorem}
Suppose that there exist $Y_f(\hat{x})$ and $Y_h(\hat{x})$ \st{}
\begin{align}
Y_f(\hat{x})\theta =& f(\hat{x},\theta) \\
Y_h(\hat{x})\theta =& h(\hat{x},\theta).
\end{align}
Let $Y(\hat{x},\hat{\theta}) = Y_f(\hat{x})-M(\hat{x},\hat{\theta})C_L(\hat{x},\hat{\theta})^{\top}Y_h(\hat{x})$ and suppose also that $\hat{\theta}$ is adaptively updated as follows:
\begin{align}
\label{estimator_adaptation}
\dot{\hat{\theta}} = (\nabla^2\psi(\hat{\theta}))^{-1} Y(\hat{x},\hat{\theta})W(\hat{x},\hat{\theta})(x-\hat{x})
\end{align}
{\color{caltechorange}($x$ is not available!!!!)} where $\psi$ is a given convex function for implicit regularization in Corollary~\ref{implicit_reg_thm}. Then $\hat{x}$ of \eqref{estimator} asymptotically converges to $x$ of \eqref{orig_dynamics_est}.
\end{theorem}
\begin{proof}
The error dynamics of $e=x-\hat{x}$ is given as follows:
\begin{align}
&\dot{e} = (A(x,\hat{x},\theta)-M(\hat{x},\hat{\theta})C_L(\hat{x},\hat{\theta})^{\top}C(x,\hat{x},\theta))e \\
&+(f(\hat{x},\theta)-f(\hat{x},\hat{\theta}))-M(\hat{x},\hat{\theta})C_L(\hat{x},\hat{\theta})^{\top}(h(\hat{x},\theta)-h(\hat{x},\hat{\theta})) \nonumber \\
&=(A(x,\hat{x},\theta)-M(\hat{x},\hat{\theta})C_L(\hat{x},\hat{\theta})^{\top}C(x,\hat{x},\theta))e-Y(\hat{x},\hat{\theta})\tilde{\theta}
\end{align}
where $\tilde{\theta}=\hat{\theta}-\theta$. Thus for a Lyapunov function given as $V=e^{\top} W(\hat{x},\hat{\theta}) e+2d_{\psi}(\theta\|\hat{\theta})$, where $d_{\psi}(\theta\|\hat{\theta})$ is the Bregman divergence $d_{\psi}(\theta\|\hat{\theta})=\psi(\theta)-\psi(\hat{\theta})+(\hat{\theta}-\theta)^{\top}\nabla\psi(\hat{\theta})$~\cite{boffi2020implicit}, the estimator \eqref{estimator} with \eqref{estimator_adaptation} gives
\begin{align}
\dot{V} =& e^{\top}(\dot{W}+2\sym(W A-C^{\top}_LC))e-e^{\top}WY\tilde{\theta}+\tilde{\theta}^{\top}YWe \nonumber \\
\leq& -2\alpha x^{\top}Wx \leq 0.
\end{align}
\end{proof}
\fi


==> sections/proof_virtual.tex <==
Let $A_{cl}=A(x,x_d,t)-B(x,t)B(x,t)^{\top}M(x,x_d,t)$. The virtual system of (\ref{adaptive_affine}), (\ref{adaptive_affine_d}), and (\ref{affine_adaptation}) with (\ref{affine_adaptive_u}), which has $(x,\hat{\theta})$ and $(x_d,\theta)$ as its particular solutions, is given as 
\begin{align}
\label{affine_q1}
\dot{q}_1 =& \dot{x}_d+A_{cl}(q_1-x_d)+B(x,t)\varphi(x,x_d,t)^{\top}(q_2-\theta) \\
\label{affine_q2}
\dot{q}_2 =& -\Gamma \varphi(x,x_d,t)B(x,t)^{\top}M(x,x_d,t)(q_1-x_d).
\end{align}
where $\tilde{\Delta}=\Delta(x,t)-\Delta(x_d,t)$ and the relation $\tilde{\Delta}^{\top}\theta=B(x,t)\varphi(x,x_d,t)^{\top}\theta$ is used. Thus for a Lyapunov function defined as $V = \delta q_1^{\top}M(x,x_d,t)\delta q_1+\delta q_2^{\top}\Gamma^{-1}\delta q_2$, we have $\dot{V} \leq -2\alpha \delta q_1^{\top}M\delta q_1+2\delta q_1^{\top}MB\varphi^{\top}\delta q_2+2\delta q_2^{\top}\Gamma^{-1}\delta \dot{q}_2$ by the proof of Theorem~\ref{modified_ncm_thm} along with the relation $\partial_{b_i(x)}M+\partial_{b_i(x_d)}M=0$. Therefore, (\ref{affine_adaptation}) gives $\dot{V} \leq -2\alpha \delta q_1^{\top}M\delta q_1$, which implies boundedness of $\delta q_1$, $\delta q_2$, $x$, and $\hat{\theta}$ as $x_d$ and $\theta$ are bounded. This also gives bounded $\delta \dot{q}_1$ due to (\ref{affine_q1}). Since $\exists \zeta(x,x_d) \succ 0$ \st{} $\dot{V}=-\delta q_1^{\top}(\zeta+2\alpha M)\delta q_1$, we have $\ddot{V}=-\delta q_1^{\top}(\dot{\zeta}+2\alpha \dot{M})\delta q_1-2\delta q_1^{\top}(\zeta+2\alpha M)\delta \dot{q}_1$, which is bounded as its arguments are all bounded. Asymptotic convergence of $\delta q$ to $0$ then follows from Barbalat's lemma~\cite{Khalil:1173048,Slotine:1228283}.
